Multi-Spacecraft Predictive Sensor Tasking for Cislunar Space Situational Awareness

This paper delves into the predictive sensor tasking algorithm for the multi-observer, multi-target sensor setting, leveraging the Extended Information Filter (EIF). Conventional predictive formulations suffer from the curse of dimensionality due to the dependence of the performance metric on the target-observer assignment history. This paper exploits the EIF's additive structure of measurement information to break the dependence and devises an efficient linear integer programming formulation. We further investigate the resulting formulation to study how the cislunar dynamics expands and shrinks the measurement information, and discuss when the information gain is maximized in relation to the observation space and the uncertainty deformation caused by the dynamics. We numerically demonstrate that the predictive sensor tasking algorithm outperforms the myopic algorithm in two different metrics, depending on the formulation.

==> text/filtering.tex <==
In this section we review the extended Kalman filter (EKF) and its information form, also known as the extended information filter (EIF)~\cite{maybeck1982stochastic, schutz2004statistical}. The EKF propagates the covariance matrix whereas the EIF propagates the inverse of the covariance matrix, which is also called the information matrix. Both algorithms approximate the nonlinear state dynamics and measurement model around a nominal state trajectory as a linear system. Although EKF and EIF are well-known algorithms, they are briefly explianed here because they form the basis of our proposed sensor tasking algorithm.
First we review the linearlized state dynamics and measurement model, followed by the prediction step and the update step of the EKF and the EIF.% in a similar manner to the review in \cite{thrun2004SimultaneousLocalizationMapping}.

\subsection{System Linearlization}
Let $\bm{x}(t)$ be the state vector and $\bm{\beta}(t)$ be the process noise assumed to be zero-mean Gaussian with covariance matrix $\tilde{\bm{Q}}(t)$. The nonlinear continuous state dynamics is given by
\begin{align}
    \bm{dx}(t) &= f(\bm{x}(t))dt + \bm{d\beta}(t)\\
    \E\left[\bm{\beta}(t)\right] &= \bm{0}, \quad \E\left[\left(\bm{\beta}(t)-\bm{\beta}(t')\right)\left(\bm{\beta}(t)-\bm{\beta}(t')\right)^T\right] = \int_{t'}^{t}\tilde{\bm{Q}}(\tau)d\tau.
\end{align}
Given a nominal trajectory $\bar{\bm{x}}(t)$, we can linearize the state dynamics around the nominal trajectory. Let $\bm{\xi}(t)=\bm{x}(t)-\bar{\bm{x}}(t)$ be the state error vector. Then, the linearized state error dynamics is given by
\begin{align}
    \label{eq:linear-dynamics}
    \bm{\xi}(t_{k}) &= \Phi(t_{k}, t_{k-1})\bm{\xi}(t_{k-1}) + \bm{w}(t_{k-1})\\
    \label{eq:stm-dynamics}
    \Phi(t_{k}, t_{k-1}) &= \int_{t_{k-1}}^{t_{k}}Df(\bar{\bm{x}}(\tau))d\tau, \quad
    \Phi(t_{k-1}, t_{k-1}) = I
\end{align}
where 
\begin{equation}
    \E\left[\bm{w}(t_{k-1})\right] = \bm{0}, \quad \E\left[\bm{w}(t_{k-1})\bm{w}(t_{k-1})^T\right] = \bm{Q}.
\end{equation}

Similarly, we can linearize the measurement model around the nominal trajectory. Let $\bm{y}(t)$ be the measurement vector and $\bm{v}(t)$ be the measurement noise assumed to be zero-mean Gaussian with covariance matrix $\bm{R}(t)$. Suppose the nonlinear measurement model is given by $\bm{y}(t) = h(\bm{x}(t))+\bar{\bm{v}}(t)$, and the deviation from the nominal measurement is denoted by $\bm{z}(t)=\bm{y}(t) - \bar{\bm{y}}(t)=\bm{y}(t) - h(\bar{\bm{x}}(t))$. Then, the linearized measurement error model is given by
\begin{align}
    \label{eq:linear-measurement}
    \bm{z}(t_{k}) &= H(t_k)\bm{\xi}(t_k) + \bm{v}(t_k)\\
    H(t_k) &= Dh(\bar{\bm{x}}(t_k)).
\end{align}
where
\begin{equation}
    \E\left[\bm{v}(t_k)\right] = \bm{0}, \quad \E\left[\bm{v}(t_k)\bm{v}(t_{k})^T\right] = \bm{R}.
\end{equation}


\subsection{Prediction Step}
The prediction step computes the prior distribution of state error before observation, $\bar{\bm{\xi}}(t_{k})$, given the previous posterior distribution of state error after observation, $\bm{\xi}(t_{k-1})$. The propagation is based on the linear dynamics of Eq. \eqref{eq:linear-dynamics}. Since the state error is assumed to be zero-mean Gaussian and independent of the process noise, the prior distribution at $t_{k}$ is also zero-mean Gaussian with covariance matrix, denoted by $\bar{\bm{P}}(t_{k})$. The prior covariance matrix $\bar{\bm{P}}(t_{k})$ and its information form $\bar{\bm{\Lambda}}(t_{k})=\bar{\bm{P}}(t_{k})^{-1}$ are computed as the sum of the linear map of $\bm{\xi}(t_{k-1})\sim\sN(\bm{0}, \bm{P}(t_{k-1}))$ and the process noise $\bm{v}(t_{k-1})\sim\sN(\bm{0}, \bm{Q})$ as follows~\cite{rencher2008linear}:
\begin{align}
    \label{eq:ekf-prediction}
    \bar{\bm{P}}(t_{k}) &= \Phi(t_{k}, t_{k-1})\bm{P}(t_{k-1})\Phi(t_{k}, t_{k-1})^T + \bm{Q}\\
    \bar{\bm{\Lambda}}(t_{k}) & = \left(\Phi(t_{k}, t_{k-1})\bm{\Lambda}^{-1}(t_{k-1})\Phi(t_{k}, t_{k-1})^T + \bm{Q}\right)^{-1}.
\end{align}
Another form of the propagation equation for the information matrix is given via Woodbury matrix identity:
\begin{equation}
    \label{eq:woodbury}
 (A+UCV)^{-1} = A^{-1} - A^{-1}U(C^{-1}+VA^{-1}U)^{-1}VA^{-1}.
\end{equation}
 Let $M=\Phi(t_{k-1}, t_{k})^T\bm{\Lambda}(t_{k-1})\Phi(t_{k-1}, t_{k})$ and substituting $A=M^{-1}$, $C=Q$, and $U=V=I$ to the identity of Eq. \eqref{eq:woodbury}, we obtain
\begin{equation}
    \bar{\bm{\Lambda}}(t_{k}) = M - M\left(Q^{-1}+M\right)^{-1}M.
\end{equation}
The propagation of the information form is computiationally less efficient than that of the covariance matrix because of the inverse operations. However, without the process noise, we obtain the following simpler linear expressions.
\begin{align}
    \label{eq:eif-prediction-noiseless}
    \bar{\bm{P}}(t_{k}) &= \Phi(t_{k}, t_{k-1})\bm{P}(t_{k-1})\Phi(t_{k}, t_{k-1})^T\\
    \bar{\bm{\Lambda}}(t_{k}) & = \Phi(t_{k-1}, t_{{k}})^T\bm{\Lambda}(t_{k-1})\Phi(t_{k-1}, t_{k})
\end{align}

\subsection{Update Step}
The update step computes the posterior distribution of state error after observation, $\bm{\xi}(t_{k})$, given the prior distribution $\bar{\bm{\xi}}(t_{k})$. The update is made to minimize the variance of the conditional distribution of $\bm{\xi}(t_{k})$ given the measurement $\bm{z}(t_{k})$ and the prior distribution $\bar{\bm{\xi}}(t_{k})$. The update in the covariance form is well-known as the Kalman filter update:
\begin{equation}
\begin{split}
    \label{eq:kalman-gain}
    \bm{P}(t_{k}) &= \left(I-\bm{K}(t_{k})H(t_{k})\right)\bar{\bm{P}}(t_{k})\\
    \bm{K}(t_{k}) &= \bar{\bm{P}}(t_{k})H(t_{k})^T\left(H(t_{k})\bar{\bm{P}}(t_{k})H(t_{k})^T + \bm{R}\right)^{-1}
\end{split}
\end{equation}
where $\bm{K}(t_{k})$ is the Kalman gain matrix. 
We can derive the update in the information form by applying the Woodbury matrix identity of Eq. \eqref{eq:woodbury} to the inverse of the covariance matrix in Eq. \eqref{eq:kalman-gain}. Substituting $A^{-1}=\bar{\bm{P}}(t_{k})=\bar{\Lambda}^{-1}(t_k)$, $C^{-1}=R$, $V=U^T=H(t_{k})$ into Eq. \eqref{eq:woodbury}, we obtain
\begin{equation}
    \label{eq:eif-update}
    \bm{\Lambda}(t_{k}) = \bar{\bm{\Lambda}}(t_{k}) + H(t_{k})^T\bm{R}^{-1}H(t_{k}).
\end{equation}
Note that the information form allows the simple additive operation for synthesizing the propagated prior information matrix $\bar{\bm{\Lambda}}(t_{k})$ and the information by the measurement $H(t_{k})^T\bm{R}^{-1}H(t_{k})$. 

\subsection{Uncertainty Propagation in EIF}
When we assume no process noise in the EIF, the combined expression of the prediction step and the update step becomes relatively simple. The uncertainty propagation of the information form is given by
\begin{equation}
    \label{eq:eif-propagation}
    \bm{\Lambda}(t_{k}) = \Phi(t_{k-1}, t_{k})^T\bm{\Lambda}(t_{k-1})\Phi(t_{k-1}, t_{k}) + H(t_{k})^T\bm{R}^{-1}H(t_{k}).
\end{equation}

This additive structure is exploited to formulate the integer linear programming problem for the predictive sensor tasking algorithm in the later section.


==> text/info_trans.tex <==
In this section, we look into the effect of the cislunar dynamics on the measurement information propagated to the evaluation time. The Fisher information matrix of Eq. \eqref{eq:eif-multi-propagation} is the sum of the information gain corresponding to each observation time, $t_L$. 
\begin{equation}
    \sum_{k=0}^{L-1}\mathcal{I}(t_{L}, t_{k}) = \sum_{k=1}^{L-1}\Phi(t_{k}, t_{L})^T H(t_{k})^T\bm{R}^{-1}H(t_{k})\Phi(t_{k}, t_{L})
\end{equation}
The information gain at each observation, $\mathcal{I}(t_{L}, t_{k})$, is the measurement information at $t_k$, which is $H(t_k)^TR^{-1}H(t_k)$, propagated to the evaluation time $t_L$. Observing $\Phi(t_{k}, t_{L})^T \Phi(t_{k}, t_{L})$ be the Cauchy-Green tensor (CGT), we can geometrically interpret $\mathcal{I}(t_{L}, t_{k})$ as the 4D ball of the measurement information at $t_k$ deformed by the CGT, which describes the backward deformation from $t_L$ to $t_k$.



==> text/linearization.tex <==
Due to the product of the covariance dynamics, our objective function is a polynomial function of the binary design variables, which are the elements of the tasking allocation matrix. To linearlize the objective function, we introduce the new variables for each product.  



==> text/system.tex <==
This section describes the cislunr system dynamics and measurement model used in this study. The cislunar dynamics is modeled as a circular restricted three-body problem (CR3BP), and we use the angle and angular rate measurements of the target space objects from the observer spacecraft based on optical sensors. The angle and angular rate measurements are often defined for the azimuth and elevation angles, but we use the directional cosines to avoid the singularity at the zenith and nadir. %PRV is also the element of the Euler parameters, also known as the quaternions, which is a common way to represent the attitude of a spacecraft. 
We derive the Jacobian of the measurement model with respect to the state of the target and the observer as well. The derivative with respect to the observer state allows us to relax the perfect knowledge assumption of the observer state, and makes the observers be one of the candidate target space objects as well. 

\subsection{System Dynamics}
We model the cislunar dynamics as a circular restricted three-body problem (CR3BP) with the Earth and Moon as the two primaries and the spacecraft as a massless particle. The CR3BP is a simplified model of the three-body problem where the mass of the smaller primary is negligible compared to the larger primary. The CR3BP is a good approximation for the translunar and cislunar regions, where the Moon is the smaller primary and the Earth is the larger primary. 
Let $\bm{r} \in \R^3$ and $\bm{v}\in\R^3$ be the nondimensionalized position and velocity of the spacecraft in the Earth-Moon rotating frame. 
The CR3BP equations of motion are given by
\begin{equation}
\dot{\bm{r}}=\bm{v}, \quad 
\dot{\bm{v}} + 2\bm{\omega}\times\bm{v} = \nabla U(\bm{r})
\end{equation}
where $\bm{\omega}=[0, 0, 1]^T$ and the potential function $U$ is given by
\begin{equation}
\begin{split}
    U &= \frac{1}{2}(x^{2}+y^{2})+\frac{1-\mu}{r_1}+\frac{\mu}{r_2}\\
    r_1^{2}&=(x+\mu)^{2}+y^{2}+z^{2}\\
    r_2^{2}&=(x-1+\mu)^{2}+y^{2}+z^{2}
    \label{eq:potential_cr3bp}
\end{split}
\end{equation}
with $\mu$ representing the mass parameter. $r_1$ and $r_2$ represent the distances from the spacecraft to Earth and Moon, respectively.

As we introduce in the next subsection, our measurement model is based on the relative state of the target and the observer. Therefore, the system state should be defined for the each target-observer pair, at least for the measurement model. Let $\bm{r}_i$ and $\bm{v}_i$ be the position and velocity of the observer $i$, and $\bm{r}_j$ and $\bm{v}_j$ be the position and velocity of the target $j$. We define the autgmented state $\bm{x}_{ij}$ for the observer $i$ and the target $j$, and the error state $\bm{\xi}_{ij}$ as follows:
\begin{equation}
    \label{eq:augmented-state}
    \bm{x}_{ij} = [\bm{r}_i^T, \bm{v}_i^T, \bm{r}_j^T, \bm{v}_j^T]^T, \quad \bm{\xi}_{ij} = \bm{x}_{ij} - \bar{\bm{x}}_{ij}
\end{equation}
where the bar denotes the nominal trajectory. Then, the error dynamics corresponding to Eq. \eqref{eq:linear-dynamics}, but without process noise, is given as follows.
\begin{equation}
    \bm{\xi}_{ijk} = \bm{\Phi}_{ij}(t_{k}, t_{k-1})\bm{\xi}_{ij, k-1}, \quad \bm{\Phi}_{ij}(t_{k}, t_{k-1}) =
    \begin{bmatrix}
        \Phi_i(t_{k}, t_{k-1}) & \bm{0}\\
        \bm{0} & \Phi_j(t_{k}, t_{k-1})
    \end{bmatrix}
\end{equation}
The state transition matrix $\Phi_i(t_{k}, t_{k-1})$ and $\Phi_j(t_{k}, t_{k-1})$ both follow the following differential equation, which corresponds to Eq. \eqref{eq:stm-dynamics}.
\begin{equation}
    \dot{\Phi}_\ell(t_{k}, t_{k-1}) =
    \begin{bmatrix}
        \bm{0} & I\\
        D\left(\nabla U(\bm{r}_\ell)\right) & L
    \end{bmatrix}, \quad
    L = \begin{bmatrix}
        0 & 2 & 0\\
        -2 & 0 & 0\\
        0 & 0 & 0
    \end{bmatrix}, \quad \forall \ell, k
\end{equation}
Although we take the augmented states for the measurements, the dynamics of the target and the observer are independent. Therefore, the computation of the state transition matrix and the state propagation are performed independently.

\subsection{Measurement Model}
We consider optical measurements of a target spacecraft from an observer spacecraft. The measurements are often defined for the azimuth and elevation angles, but instead we use the directional cosine vector and its rate to avoid the singularity at the zenith and nadir. Let $\bm{r}$ and $\bm{v}$ be the position vectors of a space object, and the subscript $i$ and $j$ denote the observer and target, respectively. The relative position and velocity vectors are given by
\begin{equation}
    \bm{r}_{ij} = \bm{r}_j - \bm{r}_i,\quad \bm{v}_{ij} = \bm{v}_j - \bm{v}_i.
\end{equation}
Our measurements are the directional cosine vector and its rate.
\begin{equation}
\bm{y}_{ij} = \frac{\bm{r}_{ij}}{\|\bm{r}_{ij}\|},\quad \dot{\bm{y}}_{ij} = \frac{\bm{v}_{ij}}{\|\bm{r}_{ij}\|} - \frac{(\bm{r}_{ij}^T\bm{v}_{ij})\bm{r}_{ij}}{\|\bm{r}_{ij}\|^3}
\end{equation}

We derive the linearlized measurement error model with respect to the error state of the target and the observer. Let $\bm{\zeta}_{ij}=\bm{y}_{ij} - \bar{\bm{y}}_{ij}$ and $\dot{\zeta}_{ij}=\dot{\bm{y}}_{ij} - \bar{\dot{\bm{y}}}_{ij}$ be the measurement error and its rate, respectively. Using the error state $\bm{\xi}_{ij}$ of Eq. \eqref{eq:augmented-state}, the linearized measurement error model is given by
\begin{equation}
    \label{eq:linear-measurement}
    \begin{bmatrix}
    \bm{\zeta}_{ij}\\
    \dot{\bm{\zeta}}_{ij}
    \end{bmatrix}
    =\bm{H_{ij}}\bm{\xi}_{ij} + \bm{v}
\end{equation}
where $H$ is the Jacobian matrix of the measurement model with respect to the state of the nominal target and the observer. $\bm{v}\sim\sN(\bm{0}, R)$ is the measurement noise.
The Jacobian matrix is given by
\renewcommand\arraystretch{1.5}
\begin{equation}
    \bm{H_{ij}} = \begin{bmatrix}
    \dfrac{\partial \bm{y}_{ij}}{\partial \bm{r}_i} & \dfrac{\partial \bm{y}_{ij}}{\partial \bm{v}_i} & \dfrac{\partial \bm{y}_{ij}}{\partial \bm{r}_j} & \dfrac{\partial \bm{y}_{ij}}{\partial \bm{v}_j}\\
    \dfrac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{r}_i} & \dfrac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{v}_i} & \dfrac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{r}_j} & \dfrac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{v}_j}
    \end{bmatrix}   
\end{equation}
where
\begin{equation}
    \begin{aligned}
        & \frac{\partial \bm{y}_{ij}}{\partial \bm{r}_i}=-\frac{\partial \bm{y}_{ij}}{\partial \bm{r}_j}=
        -\frac{\bm{I}}{\|\bm{r}_{ij}\|}+\frac{\bm{r}_{ij}\bm{r}_{ij}^T}{\|\bm{r}_{ij}\|^3}\\  
        & \frac{\partial \bm{y}_{ij}}{\partial \bm{v}_i}=-\frac{\partial \bm{y}_{ij}}{\partial \bm{v}_j}=
        \bm{0} \\ 
        & \frac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{r}_i}=-\frac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{r}_j}=
        \frac{\dot{\bm{r}}_{ij}\bm{r}_{ij}^T}{\|\bm{r}_{ij}\|^3}+\frac{\bm{r}_{ij}^T\dot{\bm{r}}_{ij}}{\|\bm{r}_{ij}\|^3}\bm{I} - 3\frac{(\bm{r}_{ij}^T\dot{\bm{r}}_{ij})\bm{r}_{ij}\bm{r}_{ij}^T}{\|\bm{r}_{ij}\|^5} \\ 
        & \frac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{v}_i}=-\frac{\partial \dot{\bm{y}}_{ij}}{\partial \bm{v}_j}=
        -\frac{\bm{I}}{\|\bm{r}_{ij}\|}+\frac{\bm{r}_{ij}\bm{r}_{ij}^T}{\|\bm{r}_{ij}\|^3}. \\ 
    \end{aligned}
\end{equation}

We assume that the measurement noise variance is fixed for the directional cosine vector, and proportional to the exposure time for the directional cosine rate. The measurement noise covariance matrix is given by
\begin{equation}
    \label{eq:obs-cov}
    R = \sigma^2 \begin{bmatrix}
    I & 0\\
    0 & \frac{2}{\Delta t^2}I
    \end{bmatrix}
\end{equation}
where $\sigma$ is the standard deviation of the angle measurement noise and $\Delta t$ is the exposure time.





